Backstepping Design of Dynamic State Feedback Controllers for Parabolic Systems

Recently, dynamic state feedback controllers that are based on dynamic extensions have been presented for heterodirectional hyperbolic systems. In this paper, a similar concept for the control of coupled diffusion-reaction systems is suggested. The introduction of a specific controller dynamics leads to homogenized diffusion coefficients for the extended system. Then, a backstepping-based static state feedback for the dynamically extended system is designed, which, overall, results in a dynamic state feedback. Such a design allows stabilizing a more general class of parabolic systems as well as assigning arbitrary closed-loop dynamics. This can be used, e.g., to achieve a decoupled input-output behavior, which is, in general, not possible with a static state feedback. A simulation example illustrates the results.

==> Usepackages.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% usepackages %%

\RequirePackage[utf8]{inputenc}

%% useful tools
\RequirePackage{ifthen}   % Load ifthen for conditional tests
\RequirePackage{version}  % include or exclude specific code

%% mathematics
\RequirePackage{amsmath,amssymb,amsfonts}
% \RequirePackage{amsthm}
\RequirePackage{siunitx}
\RequirePackage{mathtools}
\RequirePackage{fp}       % fixed point arithmetics
\RequirePackage{trfsigns} % transformation signs (e.g. Fourier)
\RequirePackage[makeroom]{cancel} % cancel mathematical expressions
\RequirePackage{etoolbox}

%% layout
\RequirePackage{caption}
\RequirePackage{subcaption}
\RequirePackage{multicol}
\RequirePackage{multirow}
\RequirePackage{tabularx}
\RequirePackage{array}
\RequirePackage[absolute,overlay]{textpos}
\RequirePackage{tabto}    % used to place symbol in margin
\RequirePackage[most]{tcolorbox}
\RequirePackage{animate}  % create animations
\RequirePackage{pifont}   % contains the symbols that are placed in the margin
\RequirePackage{graphicx}
\RequirePackage[dvipsnames,table]{xcolor}
\RequirePackage{float}
% \RequirePackage{ulem}

%% tikz
\RequirePackage{tikz}
\usetikzlibrary{arrows,arrows.meta,shapes,shapes.misc,calc}
\usetikzlibrary{positioning}
\usetikzlibrary{overlay-beamer-styles}
\usetikzlibrary{decorations.pathreplacing,decorations.markings}

% %% bibliography
% \RequirePackage[
%     backend=biber,
%     style=authoryear,
%     firstinits=true,
%     uniquename=init,
%     maxbibnames=99,
%     date=year,
%     url=false,
%     isbn=false,
%     doi=false
%   ]{biblatex}

%% quotation marks
% \RequirePackage[autostyle]{csquotes}

\RequirePackage{lipsum}
\RequirePackage{blindtext}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Colors %%

\definecolor{ovguPurpleDark}{RGB}{122,0,63}
\definecolor{ovguPurpleMedium}{RGB}{188,127,159}
\definecolor{ovguPurpleLight}{RGB}{245,235,240}
\definecolor{ovguGrey}{RGB}{111,111,111}
\definecolor{feitGreenDark}{RGB}{148,193,45}
\definecolor{feitGreenMedium}{RGB}{201,224,150}
\definecolor{feitGreenLight}{RGB}{247,250,239}

\def\mathcolor#1#{\mathcoloraux{#1}}
\newcommand*{\mathcoloraux}[3]{%
  \protect\leavevmode
  \begingroup
    \color#1{#2}#3%
  \endgroup
}
\definecolor{darkgray}{gray}{.4}
\definecolor{lightgray}{gray}{0.8}
\definecolor{myblue}{RGB}{0,167,255}
\definecolor{myorange}{RGB}{255,127,0}
\newcommand{\mathblue}[1]{\mathcolor{myblue}{#1}}
\newcommand{\mathorange}[1]{\mathcolor{myorange}{#1}}
\newcommand{\mathgreen}[1]{\mathcolor{OliveGreen}{#1}}
\newcommand{\mathgray}[1]{\mathcolor{Gray}{#1}}
\newcommand{\eqhighlight}[1]{%
  \colorbox{red!15}{$\displaystyle#1$}}
\newcommand{\mycite}[1]{\textcolor{darkgray}{\cite{#1}}}
\colorlet{darkorange}{orange!70!black}
\colorlet{lightorange}{orange!10!black}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Link symbol
\newcommand{\linksymbol}{\ding{229}~}
